LAMNER: Code Comment Generation Using Character Language Model and Named Entity Recognition

Code comment generation is the task of generating a high-level natural language description for a given code method or function. Although researchers have been studying multiple ways to generate code comments automatically, previous work mainly considers representing a code token in its entirety semantics form only (e.g., a language model is used to learn the semantics of a code token), and additional code properties such as the tree structure of a code are included as an auxiliary input to the model. There are two limitations: 1) Learning the code token in its entirety form may not be able to capture information succinctly in source code, and 2) The code token does not contain additional syntactic information, inherently important in programming languages. In this paper, we present LAnguage Model and Named Entity Recognition (LAMNER), a code comment generator capable of encoding code constructs effectively and capturing the structural property of a code token. A character-level language model is used to learn the semantic representation to encode a code token. For the structural property of a token, a Named Entity Recognition model is trained to learn the different types of code tokens. These representations are then fed into an encoder-decoder architecture to generate code comments. We evaluate the generated comments from LAMNER and other baselines on a popular Java dataset with four commonly used metrics. Our results show that LAMNER is effective and improves over the best baseline model in BLEU-1, BLEU-2, BLEU-3, BLEU-4, ROUGE-L, METEOR, and CIDEr by 14.34%, 18.98%, 21.55%, 23.00%, 10.52%, 1.44%, and 25.86%, respectively. Additionally, we fused LAMNER's code representation with the baseline models, and the fused models consistently showed improvement over the non-fused models. The human evaluation further shows that LAMNER produces high-quality code comments.

==> reviews.tex <==
Review #288A
===========================================================================

Overall merit
-------------
2. Weak reject

Paper summary
-------------
This paper focuses on the problem of automatic comment generation for methods.  Specifically, the goal is to improve upon existing deep learning approaches for generating a comment for a given Java method.  The approach is to capture each code token's syntactic role in the code and its semantics amidst identifiers composed of multiple words in the model.  The approach is compared against several state of the art deep learning approaches and an ablation study is included to evaluate the different variations of the approach, particularly using only the semantic embeddings or the syntactic embeddings.  The BLEU, ROGUE-L, METEOR, and CIDEx metrics all show this approach provides percentage improvements from 1 to 26% over state of the art deep learning approaches.

Strengths
---------
- The related work is covered well.
- The quantitative evaluation is against state of the art baselines using standard metrics.

Weaknesses
----------
- The paper has minimal, incremental novelty and significance.
- The qualitative evaluation needs more description and reporting of the ratings.  Are they averages, medians, over how much data?
- The metrics being used, while standard for deep learning, should still be described briefly and intuitively for a broader audience of readers.

Comments for authors
--------------------
Soundness:  The deep learning approach relies on existing approaches for different aspects of the overall approach, and is technically sound.  The quantitative evaluation study is sound.  The qualitative study is missing details to judge.

Significance: The additions are incremental.  The quantitative measures show good improvements; however, the qualitative data for 100 randomly sampled comment-method pairs do not show much improvement.  There is already a high level of quality for the state of the art.

Novelty: The two components that have been added are based on well known ideas that identifiers need to be split to gain their Semantics for analysis and that the structural role that an identifier plays in the code (method name, class name, variables, ...) helps in discerning more intrinsic meaning to the token.  The novelty is incremental.

Verifiability:  The work can only be verified by making the software available given how these deep learning approaches are implemented with parameterizations.  The data is a standard set.

Presentation:  Overall, the paper is organized well.  However, there is a very small amount of the paper dedicated to the new additions, 1 1/2 pages maximum.  Most of the paper is dedicated to the evaluation.  Some things are left vague, particularly the qualitative study design.  Some of the figures are quite small to read.

Questions for authors to respond to
-----------------------------------
1. What ratings are being reported for the qualitative ratings?  
2. Why not report them as box and whiskers to show the ranges?
3. What aspects of the work are really novel techniques and not known techniques applied as tweaks to existing deep learning approaches?

Comments on the author's response (FILL IN ONLY AFTER AUTHORS' RESPONSE)
------------------------------------------------------------------------
Thank you to the authors for the response to my questions.  I strongly encourage that the authors show ranges instead of averages in the final paper.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #288B
===========================================================================
* Updated: 4 Mar 2022 9:59:16pm AoE

Overall merit
-------------
3. Weak accept

Paper summary
-------------
In this paper, the authors tackle the problem of code comprehension by proposing an automated comment generation approach. Specifically, the authors propose LAMNER, a code comment generator that captures the semantics and syntactical information of code tokens (with the help of a language model and a named entity recognition model) and then passes the concatenated output embeddings to an encoder-decoder which is in charge of generating code comments.
The authors extensively evaluated their proposed framework and compared it with 7 baselines and 4+1 variants of the proposed framework. The achieved results indicate that LAMNER outperforms the state-of-the-art approaches significantly. Furthermore, the authors conduct an ablation study to learn how different features of the input (semantic or structural information) impact the performance. Finally, the authors conducted a human study to evaluate the best baseline against the proposed approach from three practical aspects (informativeness, relevance, fluency), and as results show the proposed model reaches better scores.

Strengths
---------
+ Overall, this is solid, well-thought, and motivating work.  
+ Important problem
+ Novel approach
+ The paper is packed with details
+ Extensive baselines for evaluation

Weaknesses
----------
- The approach lacks some details
- The replication package lacks documentation

Comments for authors
--------------------
# Novelty
The presented framework leverages existing state-of-the-art techniques and incorporates them to solve an existing problem with a novel and well-evaluated approach.

# Significance
The achieved results show clear evidence for progress on the state of the art and the contributions are clearly valuable.

# Soundness
- Approach: The description of the approach lacks some details and in the following, I mention the most important ones:
	1. Embeddings Concatenation: The paper doesn't provide much detail regarding how output embeddings of two models (language model + NER) are merged. Did you apply any processing for that, e.g., normalization? Also in Fig 1, the input source code goes into one component ("Pre-trained Semantic Syntax Embedding"), which doesn't specify where two embeddings are actually created and then combined.
	2. Language Model: Can you explain a bit about this sentence: "this language model can capture multiple words within a token"
	3. Semantic-Syntax Encoder: The details provided in section 2.3.1 seems limited for replication of the process. This could be addressed by the replication package, which at its current state doesn't help much.
- Training:
	1. Named Entity Recognition: Concerning the training of NER, what does "object" (line 540) refer to? Plus, I don't understand the role of NER when there is already a way to extract structural information (Javalang library)? Is NER necessary because we want to have such information embedded? or because Javalang is not helpful when it comes to incomplete code snippets? or both? Can you provide some details on that?
	2. Line 641: I didn't understand what you mean by: "the code embeddings are further fine-tuned during training"?
- Human Study:
	1. What were the criteria to filter participants? You mentioned they should "understand the generated summaries and code", but you didn't provide how this assessment is done.

# Presentation
The paper is packed with information which makes it hard to follow at different stages. Said that it is a well-written and organized paper and overall I enjoyed reading it. In the following, I bring up the main issues I encountered:
1. Introduction, lines 112-131: This section provides some examples about the two limitations, but in reality, reading the paragraphs didn't help me to understand the root issue. For instance, you refer to camel casing convention without describing what is the root issue and how your approach addresses it. Please consider revising this part.
2. Line 137: It would be helpful to provide an example of "code token structural property" here.
3. Line 164: The sentence doesn't read well.
4. Line 215: "4 and 6" -> "4 to 6"
5. There is no background information about Named Entity Recognition (NER). It's worth adding some sentences about it. This could be combined with the answer to question #2.
6. Please consider moving figures 4 and 5 closer to where they are discussed.
7. The titles of 4.1, 4.2, and 4.3 don't need the parentheses.
8. Line 882: "for each model" is misleading, as you evaluated LAMNER only against the best baseline (RENCOS).
9. Line 905: "four"->"three"


# Verifiability
The replication package at this state is not very useful, without any documentation or instructions. The README file is literally empty.

Questions for authors to respond to
-----------------------------------
# Questions
1. Can you provide some clarification concerning the concatenation of embeddings?
2. As I said in the comments section, can you provide some clarification about the role of NER (compared to using Javalang)?
3. What does "the code embeddings are further fine-tuned during training" refer to?

Comments on the author's response (FILL IN ONLY AFTER AUTHORS' RESPONSE)
------------------------------------------------------------------------
I'd like to thank the authors for addressing my concerns on the role of NER and concatenation of embeddings. The provided answer convinced me in those regards. I hope to see such additional clarifications in the revised edition.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #288C
===========================================================================

Overall merit
-------------
3. Weak accept

Paper summary
-------------
The authors present the LAnguage Model and Named Entity Recognition (LAMNER), a code comment generator capable of effectively encoding identifiers and capturing a code token’s structural property. To encode a code token that includes a type of identifier, e.g., camel case identifier, snake case identifier, etc., a character-level language model is used to learn the semantic representation. For the structural property of a token, a Named Entity Recognition (NER) model is trained to understand the code constructs. These representations (semantics-syntax embeddings) are then fed into an encoder-decoder architecture to generate code comments. To validate their work authors compared LAMNER with the 7 state-of-the-art methods using several metrics: BLEU, ROGUE-L, METEOR, and CIDEr. Results show that LAMNER improves over the best baseline model, and also can be used in combination (can be fused) with the existing techniques to improve the performance. To validate their work authors use Java source code present in existing GitHub repositories comprising 69,708 code-comment pairs.  The authors also conduct a qualitative study to evaluate the generated comments from LAMNER which states that the comments generated are quite useful for the developers. The study evaluates code comments on the basis of three metrics, viz., Informativeness, Fluency, and Relevance.

Strengths
---------
+ Paper is well-structured and well-driven with research questions. The authors have done great work in explaining the theory as well as the experimental part in a detailed manner.
+ An exhaustive comparison is presented with 7 state-of-the-art works using several metrics.
+ Fig. 1, 2, and 3 are nicely put up to explain the working procedure of the algorithms involved. 
+ Trained models are open-sourced for the replication of the results.

Weaknesses
----------
+ Fig 4 and 5 are not nicely visible and should be enlarged.
+ Conclusion and Future work could be improved.
+ The entire work could be made available as a tool for research community's use.

Comments for authors
--------------------
Soundness: State-of-the-art Machine Learning methods are used and well-explained to implement the work. Hence, the work is sound.
Significance: The automated generation of code comments is a great boon in the code review task. Hence, it is very significant.
Novelty: Combining the Syntactic and Semantic understanding of code is a novel thought and the results show that it helps in improving performance. Work is novel and helps improve the baseline's performance.
Verifiability: Authors have validated their work by comparing it with 7 existing works using several evaluation metrics. Hence, it is well-verified.
Presentation: The work is well-written and well-structured. However, some of the figures (Fig. 4 and 5) need to be enlarged.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #288D
===========================================================================

Decision recommendation
-----------------------
4. Accept

Meta-review
-----------
Congratulations on your acceptance. After careful evaluation of each other's reviews and the authors' response, the reviewers came to the conclusion that the work provides a sufficient novelty and an extensive quantitative evaluation against state-of-the-art baselines that merits acceptance.

When preparing the CR version, the reviewers strongly encourage the following changes:

- clarify the novelty of the approach (parts that are novel versus existing approaches being applied into a new context) (RA)
- clarify parts of the approach related to embeddings and training (RB)
- better describe the qualitative evaluation (RA, RB) and show ranges of values (e.g., as box and whiskers if space allows) (RA)
- provide brief definitions for the automatic evaluation metrics (RA)
- document the replication package (RB)

We trust that the authors will incorporate the above changes as well as improve other presentation aspects as suggested in the detailed comments from reviewers.


